Transwarp Conduit: Interoperable Blockchain Application Framework

Transwarp-Conduit (TWC) is a protocol for message transfers between two smart-contract enabled blockchains. Furthermore, we specify an application framework (leveraging the TWC protocol) that enables developers to define arbitrarily complex cross-blockchain applications, simply by deploying framework-compliant smart contracts and hosting a TWC node (daemon process).The TWC protocol is implementable without additional effort on part of the base blockchain protocol.

==> startuml.latex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usepackage{aeguill}
% \begin{document}
% generated by Plantuml 1.2018.14      
\definecolor{plantucolor0000}{RGB}{0,0,0}
\definecolor{plantucolor0001}{RGB}{255,255,255}
\definecolor{plantucolor0002}{RGB}{168,0,54}
\definecolor{plantucolor0003}{RGB}{254,254,206}
\definecolor{plantucolor0004}{RGB}{238,238,238}
\begin{tikzpicture}[yscale=-1
,pstyle0/.style={color=black,fill=white,line width=2.0pt}
,pstyle2/.style={color=plantucolor0002,line width=1.0pt,dash pattern=on 5.0pt off 5.0pt}
,pstyle3/.style={color=plantucolor0002,fill=plantucolor0003,line width=2.0pt}
,pstyle4/.style={color=plantucolor0002,line width=2.0pt}
,pstyle5/.style={color=plantucolor0002,fill=plantucolor0003,line width=1.5pt}
,pstyle6/.style={color=plantucolor0002,fill=plantucolor0002,line width=1.0pt}
,pstyle7/.style={color=plantucolor0002,line width=1.0pt}
,pstyle8/.style={color=black,fill=plantucolor0004,line width=1.0pt}
,pstyle9/.style={color=black,line width=2.0pt}
,pstyle10/.style={color=plantucolor0002,line width=1.0pt,dash pattern=on 2.0pt off 2.0pt}
]
\node at (541.8274pt,10pt)[below right,color=black]{\textbf{"TWC Sequence Diagram (success scenario)"}};
\draw[pstyle0] (593.7571pt,383pt) rectangle (1115.0517pt,532pt);
\draw[pstyle0] (593.7571pt,613pt) rectangle (1388.4184pt,909pt);
\draw[fill=white,color=white,line width=1.0pt] (593.7571pt,829pt) rectangle (1388.4184pt,909pt);
\draw[pstyle2] (25pt,112pt) -- (25pt,926pt);
\draw[pstyle2] (366.6411pt,112pt) -- (366.6411pt,926pt);
\draw[pstyle2] (634.7571pt,112pt) -- (634.7571pt,926pt);
\draw[pstyle2] (958.8002pt,112pt) -- (958.8002pt,926pt);
\draw[pstyle2] (1109.4774pt,112pt) -- (1109.4774pt,926pt);
\draw[pstyle2] (1302.0184pt,112pt) -- (1302.0184pt,926pt);
\node at (8pt,98pt)[below right,color=black]{User};
\draw[pstyle3] (25.8308pt,41pt) ellipse (8pt and 8pt);
\draw[pstyle4] (25.8308pt,49pt) -- (25.8308pt,76pt)(12.8308pt,57pt) -- (38.8308pt,57pt)(25.8308pt,76pt) -- (12.8308pt,91pt)(25.8308pt,76pt) -- (38.8308pt,91pt);
\node at (8pt,925pt)[below right,color=black]{User};
\draw[pstyle3] (25.8308pt,949pt) ellipse (8pt and 8pt);
\draw[pstyle4] (25.8308pt,957pt) -- (25.8308pt,984pt)(12.8308pt,965pt) -- (38.8308pt,965pt)(25.8308pt,984pt) -- (12.8308pt,999pt)(25.8308pt,984pt) -- (38.8308pt,999pt);
\draw[pstyle5] (308.6411pt,79pt) rectangle (420.9649pt,107pt);
\node at (315.6411pt,86pt)[below right,color=black]{SourceAdapter};
\draw[pstyle5] (308.6411pt,925pt) rectangle (420.9649pt,953pt);
\node at (315.6411pt,932pt)[below right,color=black]{SourceAdapter};
\draw[pstyle5] (603.7571pt,79pt) rectangle (662.8308pt,107pt);
\node at (610.7571pt,86pt)[below right,color=black]{Bridge};
\draw[pstyle5] (603.7571pt,925pt) rectangle (662.8308pt,953pt);
\node at (610.7571pt,932pt)[below right,color=black]{Bridge};
\draw[pstyle5] (917.8002pt,79pt) rectangle (996.782pt,107pt);
\node at (924.8002pt,86pt)[below right,color=black]{Signatory};
\draw[pstyle5] (917.8002pt,925pt) rectangle (996.782pt,953pt);
\node at (924.8002pt,932pt)[below right,color=black]{Signatory};
\draw[pstyle5] (1036.4774pt,79pt) rectangle (1179.626pt,107pt);
\node at (1043.4774pt,86pt)[below right,color=black]{DestinationAdapter};
\draw[pstyle5] (1036.4774pt,925pt) rectangle (1179.626pt,953pt);
\node at (1043.4774pt,932pt)[below right,color=black]{DestinationAdapter};
\draw[pstyle5] (1227.0184pt,79pt) rectangle (1374.4184pt,107pt);
\node at (1234.0184pt,86pt)[below right,color=black]{DestinationContract};
\draw[pstyle5] (1227.0184pt,925pt) rectangle (1374.4184pt,953pt);
\node at (1234.0184pt,932pt)[below right,color=black]{DestinationContract};
\draw[pstyle6] (354.803pt,137pt) -- (364.803pt,141pt) -- (354.803pt,145pt) -- (358.803pt,141pt) -- cycle;
\draw[pstyle7] (25.8308pt,141pt) -- (360.803pt,141pt);
\node at (32.8308pt,126pt)[below right,color=black]{requestTransfer(data, destAddr, gas), pay transferFee};
\draw[pstyle7] (366.803pt,168pt) -- (408.803pt,168pt);
\draw[pstyle7] (408.803pt,168pt) -- (408.803pt,181pt);
\draw[pstyle7] (367.803pt,181pt) -- (408.803pt,181pt);
\draw[pstyle6] (377.803pt,177pt) -- (367.803pt,181pt) -- (377.803pt,185pt) -- (373.803pt,181pt) -- cycle;
\node at (373.803pt,153pt)[below right,color=black]{validate user};
\draw[pstyle7] (366.803pt,208pt) -- (408.803pt,208pt);
\draw[pstyle7] (408.803pt,208pt) -- (408.803pt,221pt);
\draw[pstyle7] (367.803pt,221pt) -- (408.803pt,221pt);
\draw[pstyle6] (377.803pt,217pt) -- (367.803pt,221pt) -- (377.803pt,225pt) -- (373.803pt,221pt) -- cycle;
\node at (373.803pt,193pt)[below right,color=black]{validate transferFee};
\draw[pstyle7] (366.803pt,248pt) -- (408.803pt,248pt);
\draw[pstyle7] (408.803pt,248pt) -- (408.803pt,261pt);
\draw[pstyle7] (367.803pt,261pt) -- (408.803pt,261pt);
\draw[pstyle6] (377.803pt,257pt) -- (367.803pt,261pt) -- (377.803pt,265pt) -- (373.803pt,261pt) -- cycle;
\node at (373.803pt,233pt)[below right,color=black]{assign consecutive transferId};
\draw[pstyle7] (633.2939pt,288pt) -- (623.2939pt,284pt);
\draw[pstyle7] (633.2939pt,288pt) -- (623.2939pt,292pt);
\draw[pstyle7] (366.803pt,288pt) -- (634.2939pt,288pt);
\node at (373.803pt,273pt)[below right,color=black]{generate BridgeTransferRequested event};
\draw[pstyle7] (635.2939pt,315pt) -- (677.2939pt,315pt);
\draw[pstyle7] (677.2939pt,315pt) -- (677.2939pt,328pt);
\draw[pstyle7] (636.2939pt,328pt) -- (677.2939pt,328pt);
\draw[pstyle6] (646.2939pt,324pt) -- (636.2939pt,328pt) -- (646.2939pt,332pt) -- (642.2939pt,328pt) -- cycle;
\node at (642.2939pt,300pt)[below right,color=black]{validate BridgeTransferRequested event is finalized};
\draw[pstyle7] (635.2939pt,355pt) -- (677.2939pt,355pt);
\draw[pstyle7] (677.2939pt,355pt) -- (677.2939pt,368pt);
\draw[pstyle7] (636.2939pt,368pt) -- (677.2939pt,368pt);
\draw[pstyle6] (646.2939pt,364pt) -- (636.2939pt,368pt) -- (646.2939pt,372pt) -- (642.2939pt,368pt) -- cycle;
\node at (642.2939pt,340pt)[below right,color=black]{compute transferHash};
\draw[pstyle8] (593.7571pt,383pt) -- (666.7571pt,383pt) -- (666.7571pt,388pt) -- (656.7571pt,398pt) -- (593.7571pt,398pt) -- (593.7571pt,383pt);
\draw[pstyle9] (593.7571pt,383pt) rectangle (1115.0517pt,532pt);
\node at (608.7571pt,384pt)[below right,color=black]{\textbf{loop}};
\node at (681.7571pt,385pt)[below right,color=black]{\textbf{[for each signatory]}};
\draw[pstyle6] (947.2911pt,413pt) -- (957.2911pt,417pt) -- (947.2911pt,421pt) -- (951.2911pt,417pt) -- cycle;
\draw[pstyle7] (635.2939pt,417pt) -- (953.2911pt,417pt);
\node at (642.2939pt,402pt)[below right,color=black]{getSignature(transferHash)};
\draw[pstyle7] (959.2911pt,444pt) -- (1001.2911pt,444pt);
\draw[pstyle7] (1001.2911pt,444pt) -- (1001.2911pt,457pt);
\draw[pstyle7] (960.2911pt,457pt) -- (1001.2911pt,457pt);
\draw[pstyle6] (970.2911pt,453pt) -- (960.2911pt,457pt) -- (970.2911pt,461pt) -- (966.2911pt,457pt) -- cycle;
\node at (966.2911pt,429pt)[below right,color=black]{validate (transferHash)};
\draw[pstyle7] (959.2911pt,484pt) -- (1001.2911pt,484pt);
\draw[pstyle7] (1001.2911pt,484pt) -- (1001.2911pt,497pt);
\draw[pstyle7] (960.2911pt,497pt) -- (1001.2911pt,497pt);
\draw[pstyle6] (970.2911pt,493pt) -- (960.2911pt,497pt) -- (970.2911pt,501pt) -- (966.2911pt,497pt) -- cycle;
\node at (966.2911pt,469pt)[below right,color=black]{sign (transferHash)};
\draw[pstyle6] (646.2939pt,520pt) -- (636.2939pt,524pt) -- (646.2939pt,528pt) -- (642.2939pt,524pt) -- cycle;
\draw[pstyle10] (640.2939pt,524pt) -- (958.2911pt,524pt);
\node at (652.2939pt,509pt)[below right,color=black]{SignedHash};
\draw[pstyle7] (635.2939pt,558pt) -- (677.2939pt,558pt);
\draw[pstyle7] (677.2939pt,558pt) -- (677.2939pt,571pt);
\draw[pstyle7] (636.2939pt,571pt) -- (677.2939pt,571pt);
\draw[pstyle6] (646.2939pt,567pt) -- (636.2939pt,571pt) -- (646.2939pt,575pt) -- (642.2939pt,571pt) -- cycle;
\node at (642.2939pt,543pt)[below right,color=black]{required number of signatures collected};
\draw[pstyle6] (1098.0517pt,594pt) -- (1108.0517pt,598pt) -- (1098.0517pt,602pt) -- (1102.0517pt,598pt) -- cycle;
\draw[pstyle7] (635.2939pt,598pt) -- (1104.0517pt,598pt);
\node at (642.2939pt,583pt)[below right,color=black]{processTransfer(txnHash, destAddr, data, gas, transferId, signatures)};
\draw[pstyle8] (593.7571pt,613pt) -- (654.7571pt,613pt) -- (654.7571pt,618pt) -- (644.7571pt,628pt) -- (593.7571pt,628pt) -- (593.7571pt,613pt);
\draw[pstyle9] (593.7571pt,613pt) rectangle (1388.4184pt,909pt);
\node at (608.7571pt,614pt)[below right,color=black]{\textbf{alt}};
\node at (669.7571pt,615pt)[below right,color=black]{\textbf{[txnHash is unique]}};
\draw[pstyle7] (1110.0517pt,647pt) -- (1152.0517pt,647pt);
\draw[pstyle7] (1152.0517pt,647pt) -- (1152.0517pt,660pt);
\draw[pstyle7] (1111.0517pt,660pt) -- (1152.0517pt,660pt);
\draw[pstyle6] (1121.0517pt,656pt) -- (1111.0517pt,660pt) -- (1121.0517pt,664pt) -- (1117.0517pt,660pt) -- cycle;
\node at (1117.0517pt,632pt)[below right,color=black]{transferId equals expected Id};
\draw[pstyle7] (1110.0517pt,687pt) -- (1152.0517pt,687pt);
\draw[pstyle7] (1152.0517pt,687pt) -- (1152.0517pt,700pt);
\draw[pstyle7] (1111.0517pt,700pt) -- (1152.0517pt,700pt);
\draw[pstyle6] (1121.0517pt,696pt) -- (1111.0517pt,700pt) -- (1121.0517pt,704pt) -- (1117.0517pt,700pt) -- cycle;
\node at (1117.0517pt,672pt)[below right,color=black]{validate signatures};
\draw[pstyle6] (1290.7184pt,723pt) -- (1300.7184pt,727pt) -- (1290.7184pt,731pt) -- (1294.7184pt,727pt) -- cycle;
\draw[pstyle7] (1110.0517pt,727pt) -- (1296.7184pt,727pt);
\node at (1117.0517pt,712pt)[below right,color=black]{destAddr.call.gas(gas)(data)};
\draw[pstyle6] (1121.0517pt,750pt) -- (1111.0517pt,754pt) -- (1121.0517pt,758pt) -- (1117.0517pt,754pt) -- cycle;
\draw[pstyle10] (1115.0517pt,754pt) -- (1301.7184pt,754pt);
\node at (1127.0517pt,739pt)[below right,color=black]{function execution result};
\draw[pstyle7] (635.2939pt,781pt) -- (645.2939pt,777pt);
\draw[pstyle7] (635.2939pt,781pt) -- (645.2939pt,785pt);
\draw[pstyle7] (635.2939pt,781pt) -- (1109.0517pt,781pt);
\node at (652.2939pt,766pt)[below right,color=black]{generate Processed event};
\draw[pstyle7] (635.2939pt,808pt) -- (677.2939pt,808pt);
\draw[pstyle7] (677.2939pt,808pt) -- (677.2939pt,821pt);
\draw[pstyle7] (636.2939pt,821pt) -- (677.2939pt,821pt);
\draw[pstyle6] (646.2939pt,817pt) -- (636.2939pt,821pt) -- (646.2939pt,825pt) -- (642.2939pt,821pt) -- cycle;
\node at (642.2939pt,793pt)[below right,color=black]{validate Processed event is finalized};
\draw[color=black,line width=1.0pt,dash pattern=on 2.0pt off 2.0pt] (593.7571pt,830pt) -- (1388.4184pt,830pt);
\node at (598.7571pt,830pt)[below right,color=black]{\textbf{[txnHash has been processed]}};
\draw[pstyle7] (635.2939pt,861pt) -- (645.2939pt,857pt);
\draw[pstyle7] (635.2939pt,861pt) -- (645.2939pt,865pt);
\draw[pstyle7] (635.2939pt,861pt) -- (1109.0517pt,861pt);
\node at (652.2939pt,846pt)[below right,color=black]{generate AlreadyProcessed event};
\draw[pstyle7] (635.2939pt,888pt) -- (677.2939pt,888pt);
\draw[pstyle7] (677.2939pt,888pt) -- (677.2939pt,901pt);
\draw[pstyle7] (636.2939pt,901pt) -- (677.2939pt,901pt);
\draw[pstyle6] (646.2939pt,897pt) -- (636.2939pt,901pt) -- (646.2939pt,905pt) -- (642.2939pt,901pt) -- cycle;
\node at (642.2939pt,873pt)[below right,color=black]{validate original Processed event is finalized};
\end{tikzpicture}
% \end{document}

